Covering the Relational Join

In this paper, we initiate a theoretical study of what we call the join covering problem. We are given a natural join query instance $Q$ on $n$ attributes and $m$ relations $(R_i)_{i \in [m]}$. Let $J_{Q} = \ \Join_{i=1}^m R_i$ denote the join output of $Q$. In addition to $Q$, we are given a parameter $\Delta: 1\le \Delta\le n$ and our goal is to compute the smallest subset $\mathcal{T}_{Q, \Delta} \subseteq J_{Q}$ such that every tuple in $J_{Q}$ is within Hamming distance $\Delta - 1$ from some tuple in $\mathcal{T}_{Q, \Delta}$. The join covering problem captures both computing the natural join from database theory and constructing a covering code with covering radius $\Delta - 1$ from coding theory, as special cases. We consider the combinatorial version of the join covering problem, where our goal is to determine the worst-case $|\mathcal{T}_{Q, \Delta}|$ in terms of the structure of $Q$ and value of $\Delta$. One obvious approach to upper bound $|\mathcal{T}_{Q, \Delta}|$ is to exploit a distance property (of Hamming distance) from coding theory and combine it with the worst-case bounds on output size of natural joins (AGM bound hereon) due to Atserias, Grohe and Marx [SIAM J. of Computing'13]. Somewhat surprisingly, this approach is not tight even for the case when the input relations have arity at most two. Instead, we show that using the polymatroid degree-based bound of Abo Khamis, Ngo and Suciu [PODS'17] in place of the AGM bound gives us a tight bound (up to constant factors) on the $|\mathcal{T}_{Q, \Delta}|$ for the arity two case. We prove lower bounds for $|\mathcal{T}_{Q, \Delta}|$ using well-known classes of error-correcting codes e.g, Reed-Solomon codes. We can extend our results for the arity two case to general arity with a polynomial gap between our upper and lower bounds.

==> intro_example.tex <==
\begin{example} \label{ex:intro}
We consider a trivial join query $J = R_1$, where $R_1$ is a relation on two attributes $1$ (say ``Conference") and $2$ (say ``Year"). Here, $G$ is an edge on $1$ and $2$ and $N = 4$. In addition, we are given $\Delta = 2$. We would like to compute $\cover(G, N, \Delta)$. We show that $\cover(G, N, \Delta) $

\begin{center}
\captionof{figure}{$K_4$ - The join query}
\begin{tikzpicture}[myn/.style={circle, draw,inner sep=0.1cm,outer sep=2pt}]
\node[myn] (A) at (1.25,-1.2) {$1$};
\node[myn] (D) at (1.25, -2.75) {$4$};
\node[myn] (C) at (3.5, -2.75) {$3$};
\node[myn] (B) at (3.5, -1.2) {$2$};
\draw[line width = 2mm, magenta] (A) -- (B) node [magenta, above left = 7.5pt, sloped = 90] (TextNode) {$R_{(1, 2)}$};
\draw[line width = 2mm, orange] (B) -- (C) node [orange, above right = 7.5pt, sloped = 90] (TextNode) {$S_{(2, 3)}$};
\draw[line width = 2mm, green] (C) -- (D) node [green, below right = 12pt, sloped = 90] (TextNode) {$T_{(3, 4)}$};
\draw[line width = 2mm, blue] (D) -- (A) node [midway, blue, above left = 1pt, sloped = 90] (TextNode) {$U_{(4, 1)}$};	
\end{tikzpicture}
\end{center}

\begin{table*}
\begin{minipage}{1.0in}
	\begin{tabular}{| c | c |}
		\hline
		\rowcolor{magenta} $1$ & $2$ \\
		\hline
		\rowcolor{magenta} ICDT & $2017$ \\
		\hline
		\rowcolor{magenta} ICDT & $2018$ \\
		\hline
		\rowcolor{magenta} ICDT & $2019$ \\
		\hline
		\rowcolor{magenta} ICDT & $2020$ \\
		\hline
	\end{tabular}
\end{minipage}
\begin{minipage}{1.1in}
	\begin{tabular}{| c | c |}
			\hline
			\rowcolor{orange} $2$ & $3$ \\
			\hline
			\rowcolor{orange} $2017$ & Europe \\
			\hline
			\rowcolor{orange} $2018$ & Europe  \\
			\hline
			\rowcolor{orange} $2019$ & Europe \\
			\hline
			\rowcolor{orange} $2020$ & Europe\\
			\hline
	\end{tabular}
\end{minipage}
\begin{minipage}{1.5in}
	\begin{tabular}{| c | c |}
			\hline
			\rowcolor{green} $3$ & $4$ \\
			\hline
			\rowcolor{green} Europe & Austria \\
			\hline
			\rowcolor{green} Europe & Denmark \\
			\hline
			\rowcolor{green} Europe & Italy \\
			\hline
			\rowcolor{green} Europe &  Portugal \\
			\hline
	\end{tabular}
\end{minipage}
\begin{minipage}{1.0in}
	\begin{tabular}{| c | c |}
		\hline
		\rowcolor{blue} $4$ & $1$ \\
		\hline
		\rowcolor{blue} Austria & ICDT\\
		\hline
		\rowcolor{blue} Denmark & ICDT\\
		\hline
		\rowcolor{blue} Italy & ICDT\\
		\hline
		\rowcolor{blue} Portugal &  ICDT\\
		\hline
	\end{tabular}  
\end{minipage}
\caption{\yell{needs to be filled in.}}
\end{table*}

\begin{table*}[!hbt]
\centering
\begin{tabular}{ll}

\begin{tabular}{| c | c | c | c |}
		\hline
		\rowcolor{violet} $1$ & $2$ & $3$ & $4$ \\
		\hline
		\rowcolor{violet}  ICDT & $2017$ & Europe & Austria \\
		\hline
		\rowcolor{violet}  ICDT & $2017$ & Europe & Denmark \\
		\hline
		\rowcolor{violet}  ICDT & $2017$ & Europe & Italy \\
	\hline
			\rowcolor{violet}  ICDT & $2017$ & Europe & Portugal \\
	\hline
		\rowcolor{violet}  ICDT & $2018$ & Europe & Austria \\
\hline
\rowcolor{violet}  ICDT & $2018$ & Europe & Denmark \\
\hline
\rowcolor{violet}  ICDT & $2018$ & Europe & Italy \\
\hline
\rowcolor{violet}  ICDT & $2018$ & Europe & Portugal \\
\hline
	\rowcolor{violet}  ICDT & $2019$ & Europe & Austria \\
\hline
\rowcolor{violet}  ICDT & $2019$ & Europe & Denmark \\
\hline
\rowcolor{violet}  ICDT & $2019$ & Europe & Italy \\
\hline
\rowcolor{violet}  ICDT & $2019$ & Europe & Portugal \\
\hline
		\rowcolor{violet}  ICDT & $2020$ & Europe & Austria \\
\hline
\rowcolor{violet}  ICDT & $2020$ & Europe & Denmark \\
\hline
\rowcolor{violet}  ICDT & $2020$ & Europe & Italy \\
\hline
\rowcolor{violet}  ICDT & $2020$ & Europe & Portugal \\
\hline
\end{tabular}

\begin{tabular}{| c | c | c | c |}
	\rowcolor{red} $1$ & $2$ & $3$ & $4$ \\
	\hline
			\rowcolor{red}  ICDT & $2017$ & Europe & Italy \\
			\hline
			\rowcolor{red}  ICDT & $2018$ & Europe & Austria \\
			\hline
			\rowcolor{red}  ICDT & $2019$ & Europe & Portugal \\
			\hline
			\rowcolor{red}  ICDT & $2020$ & Europe & Denmark \\
			\hline
\end{tabular}

\end{tabular}
\caption{\yell{needs to be filled in}}

\end{table*}
\end{example}

==> lower_bound_general_arity.tex <==
\subsection{Lower Bound} \label{galb}
In this section, we prove a lower bound for the gap between $LP_{ub}(G, k)$ and $LP_{lb}(G, k)$. The interesting aspect of this result is to show that some multiplicative factor is necessary in Theorem~\ref{generalarityubtheorem}. The necessity of the additive factor is proved for the case when $G$ has only edge $e = V$ and $k = 1$.
\begin{theorem} \label{thm:lbga1}
There exists an instance \\$G' = (V', E')$ such that for $k = \Theta(n/\log{n})$:
\[\dfrac{LP_{ub}(G, k)}{LP_{lb}(G, k)} \ge 1 + 1/\tilde{e} - \delta,\]
where $\delta$ is a constant $> 0$.
\end{theorem}		
We will need the following set cover instance for our proof:
\begin{lemma}
\label{lemma:set-cover-gap}
For a large enough constant $C > 0$ the following is true. Let $\epsilon > 0$ be a small enough constant.  Then for every large enough integer $n$, there is a graph $G = (V, E)$ ($|V| = [n]$, $E = \{E_1, E_2, \dots, E_n\}$) and an integer $d  = \ceil{\frac{C\ln n}{\eps^2}}$ such that:
\begin{enumerate}[label=(\ref{lemma:set-cover-gap}\alph*), itemsep=0pt, leftmargin=*]
\item For every $i \in [n]$, we have $|E_i| \leq (1+\eps)d$; \label{property:set-cover-s-degree}
\item For every $v \in V$, we have $\|\{{i \in [n]: v \in E_i}\}| \geq (1-\eps)d$;  \label{property:set-cover-v-degree}
\item For every $\alpha \in  [0, 2]$ and every $I \subseteq V$ of size at most $\alpha  n/d$, we have $\left|\union_{i \in I}E_i \right| \leq (1-e^{-\alpha} + \epsilon) n$. \label{property:set-cover-gap}
\end{enumerate}
\end{lemma}
The proof is in Appendix~\ref{set-cover-gap-proof}.
			
We now prove Theorem~\ref{thm:lbga1}. To this end, we first construct the lower bound instance to obtain the required gap. Let $\eps > 0$ be an arbitrary constant. Construct a graph $G = (V, E)$ ($|V| = |E| = t, E = \{E_1, E_2, $\\$\dots, E_t\}$) and integer $d$ using Lemma~\ref{lemma:set-cover-gap}.  We now create a new graph $G' = (V', E')$, which is the instance that we be would working with for the remaining of this proof, as follows. We initially assign $V' = V$ (assuming that the vertices are indexed from $1$ to $t$) and $E' = E$. We add $td'$ more vertices to $V'$ (i.e. $|V'| = t + d't$), where $d' = \floor*{(1-1/\tilde{e})d}$. For each $E'_i \in E'$, we expand it by adding the first $d'$ vertices (`private' vertices of $E'_i$) that have been not picked by any other edge $E'_j \in E'$ in the range $[t + 1, t+d't]$. Let $k = (2-1/\tilde{e})t$. We do this argument in two steps - we first upper bound $LP_{lb}(G, k)$ and then lower bound $LP_{ub}(G, k)$. This is sufficient to lower bound $LP_{ub}(G, k)/LP_{lb}(G, k)$.
			
To cover $k$ vertices fractionally, for each edge $E'_i \in E'$, we let $x_{E'_i} = \frac{1}{(1-\eps)d}$. Further, the number of sets in which each vertex $j \in [t]$ is contained in at least $(1 - \eps)d$ edges (by Property~\ref{property:set-cover-v-degree}). In particular, this implies $z_{v} = \sum_{E'_i \ni v}x_{E'_i} \ge 1$ for every $v \in [t]$. As a result, by picking all the $t$ hyper-edges, $\sum_{v \in [t]}z_{v} \ge t$ and we can set $z_{v} = 1$ for all $v \in [t]$. For all $v \in (t, t+d't)$, we have $z_{v} = \frac{1}{(1-\eps)d}$ since they are incident to only one edge. Further, by picking the $t$ hyper-edges we have also ended up covering $\frac{td'}{(1-\eps)d} \geq (1-1/\tilde{e})t$ fractional vertices in $(t, t+d't]$. Thus, overall, we can cover $t + (1-1/\tilde{e})t = k$ vertices and $LP_{lb} \le t/(1 - \eps)d$.

We now cover $k$ vertices integrally and show that we need at least $(1+1/\tilde{e} - 3\eps)t/d$ fractional edges. The proof is by contradiction. We start by assuming that there exists a pick with $\alpha t/d$ integral hyper-edges and $\beta t/d$ fractional hyper-edges such that $\alpha + \beta < 1+1/\tilde{e}-3\eps, \alpha > 0, \beta > 0$ to cover $k$ vertices integrally. Note that using $\alpha t/d$ integral edges we can cover $ \le (1 - \exp(-\alpha) + \eps)t$ vertices from $[t]$ (by Property~\ref{property:set-cover-gap}) and $\alpha (t/d) d'$ vertices from $(t, t + td']$. The $\beta (t/d)$ fractional hyperedges can cover at most $\beta (t/d) (1 + \eps)d$ vertices from $[t]$ and no `private' vertex is covered by any of them. Thus, in total we have covered
\begin{align*}
(1-\exp(-\alpha) + \eps)t + \alpha(t/d) d' + \beta (t/d) (1+\eps)d \numberthis \label{eq:lbagm1}
\end{align*}
vertices. (In Appendix ~\ref{lbga1calc}, we will show that this is $<k$.) Finally, we have proved that we need 
\[LP_{ub} (G, k) \ge (1 + 1/\tilde{e} - 3\eps) t/d.\]
Hence, we have
\begin{align*}
\dfrac{LP_{ub}(G, k)}{LP_{lb}(G, k)} & \ge \dfrac{(1 + 1/\tilde{e} - 3\eps)}{(1 - \eps)} \\ 
&\ge 1 + 1/\tilde{e} - 4\eps = 1 + 1/\tilde{e} - \delta, 
\end{align*}
where the last equality follows from setting $\eps = \delta/4$. This completes the proof.


==> results_table.tex <==
\begin{table*}[th!]
	{\small
	\centering
	{
		\hspace{0.5cm} {
	\begin{tabular}{| c | c | c | c|}
		\hline
	\end{tabular}}
	\caption{\yell{needs to be filled in}} \label{tab:intro_results}
}
}
\end{table*}
